DART: A Compact Platform For Autonomous Driving Research

This paper presents the design of a research platform for autonomous driving applications, the Delft's Autonomous-driving Robotic Testbed (DART). Our goal was to design a small-scale car-like robot equipped with all the hardware needed for on-board navigation and control while keeping it cost-effective and easy to replicate. To develop DART, we built on an existing off-the-shelf model and augmented its sensor suite to improve its capabilities for control and motion planning tasks. We detail the hardware setup and the system identification challenges to derive the vehicle's models. Furthermore, we present some use cases where we used DART to test different motion planning applications to show the versatility of the platform. Finally, we provide a git repository with all the details to replicate DART, complete with a simulation environment and the data used for system identification.

==> sections/temporary_notes.tex <==
\section{Temporary notes to self}
\begin{itemize}
    \item \textbf{main features}: very cheap, easy to modify (since very little custom parts), quite versatile in applications due to connectivity and racing asset. Areas of research we have used them for: Autonomous driving (MPCC experiments), System identification with machine learning (GPs), Platooning.
    
    \item \textbf{hardware modifications} starting from base kit describe enhancements. Magnet sensor, arduino, IMU, lidar, external battery pack, new servomotor. PVC plates, metal rings to increase spring preload and building scheme, also IMU little house. 
    
    \item \textbf{System identification}: Kinematic bicycle model: Steering curve, with delay identification, throttle curve (This can be done without motion capture system). Dynamic bicycle model and GPs (needs motion capture system) for more aggressive manoeuvres. [Here I would just put the simplest model fitting with GPs]

    \item \textbf{Multi-robot experiments}: Lidar-based localization, and information sharing over the wifi. Show linear controller platooning results. [About the camera we can just say that we left it as it is. If now mention that we also used Apriltag but I would need to talk to Thijs about putting it back in the repo]


    \item \textbf{Literature review}: Consisting mainly of comparable robotic platform we can recycle some info from Thijs theisis. Maybe check that the prices ecc are still correct, and check if some other platforms have come about. Maybe add a row in the table saying what kind of experiments they were used for. Maybe we can ask Thijs to help with this.
    \item \textbf{Questions}: how long does the paper need to be? Do we have to submit a video too? When? 

    \item \textbf{Sust out git repo}: Sust out the safety business. Also prepare a vref-steer angle controlled racecar. Also sust out the gamepad not working without a monitor. Also change name and iclude simulator and model fitting results. include build manual. Add PVC plates cad files
\end{itemize}

